Making Paper Reviewing Robust to Bid Manipulation Attacks

Most computer science conferences rely on paper bidding to assign reviewers to papers. Although paper bidding enables high-quality assignments in days of unprecedented submission numbers, it also opens the door for dishonest reviewers to adversarially influence paper reviewing assignments. Anecdotal evidence suggests that some reviewers bid on papers by "friends" or colluding authors, even though these papers are outside their area of expertise, and recommend them for acceptance without considering the merit of the work. In this paper, we study the efficacy of such bid manipulation attacks and find that, indeed, they can jeopardize the integrity of the review process. We develop a novel approach for paper bidding and assignment that is much more robust against such attacks. We show empirically that our approach provides robustness even when dishonest reviewers collude, have full knowledge of the assignment system's internal workings, and have access to the system's inputs. In addition to being more robust, the quality of our paper review assignments is comparable to that of current, non-robust assignment approaches.

==> sections/attack.tex <==
\section{Cheating}

The primary goal of a cheating reviewer is to manipulate the paper assignment algorithm and secure an outcome that is favorable for her. We make the following assumptions on the adversary's capabilities:

\begin{enumerate}[1.]
\item The adversary belongs to a colluding group of $M_c \geq 1$ reviewers in an attempt to secure the target paper assignment. One possible scenario is that the reviewer is asked by the target paper's author to secure the assignment, and she contacts a group of friends to collectively bid on the paper to maximize their chances.
\item The adversary would have obtained a rank of $K$ or lower if her bid had been genuine. This assumption distinguishes the situation of an adversarial reviewer that attempts to cheat the system from a legitimately qualified reviewer.
\end{enumerate}

\subsection{Cheating Methods}
\label{sec:cheating}
\paragraph{White-box cheating.}
For our setting of using bids predicted by the linear regression model in Section \ref{sec:model} as input for the assignment algorithm, the white-box setting assumes that the adversary knows $X$ and $y$ in advance and can select the colluding group and decide how to bid based on these information.

Note that both the linear regression and the assignment algorithm are deterministic and there are only finitely many choices a reviewer $r$ can make regarding a paper $p$, namely the collusion group and their bids. However, it's still intractable to optimize among these choices to guarantee that $r$ gets paper $p$ because of the large size of possible choice space -- $\binom{m_1-1}{L_c} * \left( \sum_{i=0}^{U}\sum_{j=0}^{U}\frac{n!}{i!j!(n-i-j)!} \right)$ -- and the complicated mapping from predicted bids scores to the final assignment.

Instead, we relax the adversary's optimization problem to maximizing their predicted score for the target paper. The intuition of this objective is that
\begin{enumerate}[1.]
\item Maximizing the predicted score for pair $(p, r)$ (our replaced object) has a high correlation with maximizing the difference between the predicted score of $(p, r)$ and others predicted score (\emph{event A}). Notice that they are not equivalent because when the adversary and her colluding group change their bidding vectors, the learned linear function from regression model will change so that not only the score of $(p, r)$ but scores of all pairs will be changed.
\item The final goal that $r$ can get paper $p$ has high a correlation with \emph{event A} under the our assignment algorithm.
\end{enumerate}

We state this relaxed objective formally: given the feature vector $X_{p,r}$ for a paper $p$ and reviewer $r$, the predicted relevance score is $$X_{p,r} w^* = X_{p,r} H^{-1} X^\top y,$$ where $y = [y_1 | y_2 | \cdots | y_{m_1}]$ is the training label vector consisting of positive, negative, and null bids, and $H = X^\intercal X + \lambda I$ is the Hessian matrix. For a non-colluding attack, the cheating reviewer may change $y_r$ arbitrarily to $y_r'$ and seek to maximize the relevance score. For an $L_c$-colluding attack, additional $L_c$ training labels $y_{s_1}, \ldots, y_{s_{L_c}}$ associated with the colluding group $S=\{s_1, \ldots, s_{L_c}\}$ may also be modified to $y_{s_1}', \ldots, y_{s_{L_c}}'$ in an attempt to maximize $r$'s score. Then the maximization problem can be stated as follows:
\begin{equation}
\label{equ:wb_obj}
    \max_{S\subseteq [m]: |S|=L_c; \forall s\in S\cup\{r\}, y_s'\in C} X_{r, p}H^{-1}\left(X_{S\cup \{r\}}^\top y_{S\cup \{r\}}' + X_{-S\cup \{r\}}^\top  y_{-S\cup \{r\}}\right),
\end{equation}
where $C=\{v\in \{-3, -1, 3\}^n \text{: both the number of -3 and 3 occur at most $U$ times in $v$}\}$. Although this optimization problem is associated with solving integer linear programming given the group $S$ and finding an optimal collusion group over all possible groups, we can solve this problem efficiently in $O(m(n\log U + \log(L_c+1)))$ time if $X_{r, p}H^{-1}X^\top $ is pre-computed. We leave the detailed solution for the appendix \todo{}.

\paragraph{Black-box cheating.}
The white-box setting assumes that an adversarial reviewer has access to the features and bids of all reviewers -- a highly unlikely scenario. In addition, we propose the following heuristic cheating method under the black-box setting when the adversarial reviewer can only know and influence the bids of herself and her collusion group.
\begin{enumerate}
	\item Choose $L_c$ reviewers most similar to $r$ as her collusion group. We can measure the similarity of two reviewers by the inner product between reviewer-related features from these two reviewers. In realistic settings, this can be done by forming a colluding group of reviewers with similar background.
	\item $r$ and reviewers in the selected collusion group give the largest bid scores to the target paper $p$ and other $U-1$ most similar papers. Similarity between papers is measured by the inner product between paper-related feature vectors from two papers. In realistic settings, this can be done by comparing the titles and abstracts of relevant papers. The remaining papers are given null bids.
\end{enumerate}
The intuition of this strategy is that if the bids for the reviewer-paper pairs, whose features are close to $(r, p)$, are large, then the model will tend to predict a high score for $(r, p)$. \cg{derive this mathematically?}

\paragraph{Comparison between different cheating methods.}
Although we can't say which method will help adversaries the most theoretically because of complicated mapping from bidding label scores to the final assignment, the analysis in the beginning of white-box cheating's introduction shows that except the exhausting enumeration of all possible choices, white-box cheating we propose is what the most adversaries can make. We may expect that white-box cheating has the largest power among all feasible cheating methods. In the experiment section we also consider several other cheating methods (\todo{for example randomly select the collusion group}). We evaluate different cheating methods to see how many chances they may improve if a random reviewer $r$ targets any paper $p$ (under some given distribution over reviewers and papers) in the experiment section. Briefly, both white-box cheating and \todo{some black box cheating} can make some adversaries to get their target papers. Moreover, the white-box cheating has the largest improvement of chances for adversaries, which is in our expectation.

Furthermore, once we consider detection in our algorithm, we also evaluate detection, which will be proposed in next section, for all cheating methods we have. It's not sufficient to only evaluate white-box cheating, since the largest power of cheating is not equivalent to the largest power of cheating under the same detection. In the experiment section, we verify that white-box cheating is still the most powerful under the detection among all cheating methods (\todo{?}) and on the other hand our detection methods have good detection performance against all proposed cheating methods.


==> sections/detection.tex <==
\section{Adversarially Robust Paper Assignment}
\label{sec:detection}

%In this section we will propose a unified framework of detection with two different detection criteria. Under this detection framework, cheating pairs detected by criterion will never get into the final assignment.
%\paragraph{Unified detection framework.}

\begin{algorithm}[!t]
\label{alg:framework}
\SetAlgoLined
\begin{algorithmic}[1]
 \STATE Predict relevance scores for all reviewer-paper pairs by $X(X^\top X + \lambda I)^{-1}X^\top \by$\;
 \STATE For each paper $p$, populate the reviewer candidate set by choosing the top-$K$ reviewers according to the predicted relevance score\;
 \STATE Run detection criterion for every pair $(r, p)$ in the candidate set and if the output is \textit{true}, remove this pair from candidate set\;
 \STATE Run the assignment algorithm among the remaining candidates and output the assignment.
 \end{algorithmic}
 \caption{Framework for adversarially robust paper assignment}
 \end{algorithm}

Given the limitation of our relevance scoring model against colluding label-poisoning attacks, we propose an additional component in our robust assignment framework that detects and rectifies training points that have disproportional influence on the model's prediction. Algorithm \ref{alg:framework} gives an overview of our robust assignment strategy.

We first limit the set of reviewer-paper pairs under consideration during the assignment phase to only the top-$K$ reviewers per paper. We will refer to this collection of reviewer-paper pairs as the \emph{candidate set}. In practice, this restriction will not affect the assignment quality since reviewers that are ranked lower are rarely given assignments.

For each pair $(r,p)$ in the candidate set, the predicted relevance score (\emph{cf.} Equation \ref{eq:relevance}) can be influenced by a malicious set of reviewers $\calM$ with $r \in \calM$ and the honest set $\calM^c$, which gives us a decomposition of the predicted score:
\begin{equation}
\label{eq:bid_partition}
s_{r,p} = X_{r,p} H^{-1} (X_\calM^\top \by_\calM + X_{\calM^c}^\top \by_{\calM^c}).
\end{equation}
Suppose that we can determine the malicious reviewers in $\calM$ as well as their (unobserved) honest bids $\tilde{\by}_\calM$. We can then easily re-compute the benign relevance scores $\tilde{s}_{r,p}$ by replacing $\by_\calM$ with $\tilde{\by}_\calM$ in Equation \ref{eq:bid_partition}. If the rank of the benign score $\tilde{s}_{r,p}$ for paper $p$ is lower than $K$, we can then determine that in a hypothetical scenario where every reviewer in $\calM$ had bid honestly, the pair $(r,p)$ would not have belonged to the candidate set. Our framework can then remove all such pairs from the candidate set and proceed with running the assignment algorithm on the remaining candidates.

However, since this malicious set and the honest bids cannot be observed, we must resort to searching for potential malicious reviewers and determining whether their observed bids have been manipulated to artificially increase the relevance score $s_{r,p}$. We give two heuristic approaches for estimating $\calM$ and $\tilde{\by}_\calM$ below.

%We propose a cheating reviewer detection algorithm that is embedded in our bid prediction and paper assignment framework (Algorithm \ref{algo:fram}). Since the assignment algorithm seeks to maximize the predicted relevance score for every paper, we may restrict it to only consider the top $K$ reviewers instead. Thus, the candidate set initially consists of all reviewer-paper pairs $(r,p)$ for which $r$ ranks in the top-$K$ for paper $p$. Now, for an adversarial reviewer $r$ who changes her bids to target paper $p$, there are two scenarios for the pair $(r, p)$ after her malicious bidding.
%\begin{enumerate}
%\item Her rank for paper $p$ is still lower than $K$. In this case, because our assignment only consider the top $K$ reviewers for each paper, she won't get this paper naturally.
%\item Her rank gets into top $K$, then we will run our detection criterion on $(r, p)$ in line 3 of algorithm \ref{algo:fram}. If our detection criterion detects it as cheating then we will remove $(r,p)$ from the candidate set.
%\end{enumerate}

%Embedded in this framework, we only need to design our detection criterion for top $K$ reviewers of each paper. Specifically, given $r$ who is already top  $K$ for paper $p$, our detection criterion should decide whether she is an adversary for $p$ or not.

\paragraph{Maximum influence.} We first consider a very aggressive heuristic, called \emph{\critonelong{}}, that seeks to find \emph{any} group of reviewers with a pre-determined size $M_d$ such that, upon manipulation of the observed bids $\by_\calM$, will cause $r$ to drop out of the top-$K$ candidate set. Mathematically, this heuristic amounts to solving the following optimization problem:
\begin{equation}
\label{eq:dwc_obj}
s_{r,p}^* = \min_{(\calM, \by_\calM') \in \calP(r, M_d)} X_{r,p} H^{-1} (X_\calM^\top \by_\calM' + X_{\calM^c}^\top \by_{\calM^c}).
\end{equation}
The underlying principle for this heuristic is that if there exists a group of malicious reviewers $\tilde{\calM}$ containing $r$ with $|\tilde{\calM}| \leq M_d$ with associated unobserved honest bids $\tilde{\by}_{\tilde{\calM}}$ then
\begin{equation}
s_{r,p}^* \leq X_{r,p} H^{-1} (X_{\tilde{\calM}}^\top \tilde{\by}_{\tilde{\calM}} + X_{\tilde{\calM}^c}^\top \by_{\tilde{\calM}^c}) = \tilde{s}_{r,p},
\label{eq:mi_bound}
\end{equation}
thus the white-box attack in section \ref{sec:cheating} will always be detected if $M_c \leq M_d$. Computation of the minimum in (\ref{eq:dwc_obj}) is analogous to solving the optimization problem in (\ref{eq:wb_obj}), and hence can also be done efficiently. Solutions for the different pairs in the candidate set can be computed in parallel for each of the $Kn$ candidates.

\begin{comment}
In principal, if $r$ is a cheating reviewer and should be ranked lower than $K$ when her bids and her colluding group's bids are genuine, then there exists such a group when $L_c \leq L_d$. Thus the true positive rate of this detection criterion is 1 for the attacks defined in section \ref{sec:cheating}. The critical trade-off is that the criterion will find many false positives, and thus can remove many legitimate reviewers from the candidate set.

%exists answer of this question is true supported by this colluding group and their (unknown to us) benign bids. Therefore if we have a black box -- given a pair $(r, p)$, output the answer of this question, we can use this black box as our criterion and it will identify all adversaries, whose rank is lower than $K$ when they bid genuinely, as cheaters. In the other word, the true positive rate is $1$ over the class of adversaries defined in the beginning of .

Similar to the white-box cheating formulation, it is intractable to optimize the rank over a large number of possible colluding groups and the integer constraints. Instead, we again relax the optimization problem to minimizing the predicted scores for a given $(p, r)$. Formally, we design the following detection criterion if the largest size of collusion group we want to detect is $L_d$:
\begin{enumerate}
	\item Solve the minimization problem:
	\begin{equation}
  \small
	\label{equ:dwc_obj}
    	\displaystyle S^*, y_{S^{*}\cup\{r\}}^* = \argmin_{S\subseteq [m]: |S|=L_d; \forall s\in S\cup\{r\}, y_s'\in C} X_{r, p}H^{-1}\left(X_{S\cup \{r\}}^\top y_{S\cup \{r\}}' + X_{-S\cup \{r\}}^\top  y_{-S\cup \{r\}}\right),
	\end{equation}
	\item Replace the bidding labels for $S^*\cup \{r\}$ by $y_{S^*\cup\{r\}}^*$ which leads to a new linear model with $$w_{detect} = H^{-1}\left(X_{-S^*\cup \{r\}}^\top y_{-S^*\cup \{r\}} + X_{S^*\cup \{r\}}^\top y_{S^*\cup \{r\}}^*\right).$$
	\item Predict scores by $w_{detect}$. If under current linear model reviewer $r$'s rank is lower than $K$, then output \textit{true}. Otherwise, output \textit{false}.
\end{enumerate}

This detection criterion can't theoretically guarantee that the adversary, whose rank should be lower than $K$ if she bids genuinely, will be detected. However, this detection criterion could give us a weaker guarantee: When $L_d \geq L_c$, the score for $(r, p)$ predicted by $w_{detect}$ is no larger than the score of $(r, p)$ when $r$ and her collusion group had not bid maliciously. Because larger scores and higher ranks have high correlation, if $r$ should have been ranked lower than $K$, the rank of $r$ under $w_{detect}$ will most likely be lower than $K$. Our proposed detection will detect $r$ as the cheater and output \textit{true} then. We formally state this weak guarantee in the following claim.

\begin{claim}
	$X$ and $y$ are observed data. Reviewer $r$ and some unknown colluding group $S_c$ ($|S_c|=L_c$) may or may not make cheating together for $r$ on $p$. Denote $y_{S_c\cup\{r\}}^{g}$ as the genuine scores that reviewers in $S_c\cup\{r\}$ would give for labels, which is unknown to us, and moreover the unknown benign linear model is $w_{b} = H^{-1}\left(X_{-S_c \cup \{r\}}^\top y_{-S_c \cup \{r\}} + X_{S_c \cup \{r\}}^\top y_{S_c\cup \{r\}}^g\right)$. Then if we have $L_d\geq L_c$
	$$
	X_{r, p}w_{detect} \leq X_{r, p}w_{b}.
	$$
\end{claim}
\end{comment}

\paragraph{Neutral preference.} The \critonelong{} heuristic can be seen as a very aggressive and loose estimate of the true score $\tilde{s}_{r,p}$ via Equation \ref{eq:mi_bound}. It is easy to see that as the number of suspected colluders $M_d$ grows large, the gap between the estimated true score $s_{r,p}^*$ and the unobserved score $\tilde{s}_{r,p}$ increases. This will cause the detection algorithm to remove many legitimate reviewers from the candidate set due to severely overestimating their potential to cheat.

We propose an alternative heuristic, called \emph{\crittwolong{}} (\crittwoshort{}), that estimates the unobserved bids $\tilde{s}_{r,p}$ from training data. For any group of reviewers $\calM$ with associated honest bids $\tilde{y}_\calM$, let $$\tilde{\bw} = H^{-1} (X_\calM^\top \tilde{\by}_\calM + X_{\calM^c}^\top \by_{\calM^c})$$ be the model trained on the unobserved bids. We define the \crittwolong{} model: $$\bw_\text{\crittwoshort{}}^{\calM} = H^{-1} (X_\calM^\top (-\mathds{1}) + X_{\calM^c}^\top \by_{\calM^c}),$$ which corresponds to replacing all bids for all reviewers in $\calM$ to the neutral bid $-1$. Intuitively, we rely on the stability of the learning algorithm for the scoring model to assert that $\bw_\text{\crittwoshort{}}^{\tilde{\calM}} \approx \tilde{\bw}$ where $\tilde{\calM}$ is the ground truth colluding party. We can then lower bound $\tilde{s}_{r,p} = X_{r,p} \tilde{\bw}$ by solving the following optimization problem:
\begin{align}
    s_{r,p}^\dagger &= \min_{\calM \subseteq \calR: r \in \calM, |\calM|=M_d} X_{r,p} H^{-1} (X_\calM^\top (-\mathds{1}) + X_{\calM^c}^\top \by_{\calM^c}) \label{eq:dud_obj} \\
    &\leq X_{r,p} \bw_\text{\crittwoshort{}}^{\tilde{\calM}} \approx \tilde{s}_{r,p}. \label{eq:np_bound}
\end{align}

\cg{consider changing this to removal and prove something using stability}

\begin{comment}
Although the \emph{worst case} detection criterion can detect almost all adversaries, it suffers the drawback of being too aggressive and removing a large number of legitimate reviewers from the candidate set. This is caused by the large gap between $X_{r, p}w_{detect}$ and $X_{r, p}w_{b}$, which calls for a tighter estimate for $X_{r, p}w_{b}$.

One natural choice is using $w_{b, undo} = H^{-1}\left(X_{-S_c \cup \{r\}}^\top y_{-S_c \cup \{r\}} + X_{S_c \cup \{r\}}^\top (-\mathds{1})\right)$ to approximate $w_{b}$, where $\mathds{1}$ is an all one vector. In $w_{b, undo}$ we undo the positive bids and negative bids from $S_c\cup \{r\}$, i.e. pretend that reviewers in $S_c\cup \{r\}$ only have null bids. This operation is approximate to removing those reviewers from the dataset. By comparing $w_{b, undo}$ and $w_{b}$, the difference is that we use $-\mathds{1}$ in $w_{b, undo}$ to replace $y_{S_c\cup \{r\}}^g$ in $w_{b}$. We can expect the difference between them will be relatively small: a genuine bid vector $y_{S_c\cup \{r\}}^g$ will tend to be consistent with the prediction on $S_c\cup \{r\}$ from the dataset excluding $S_c\cup \{r\}$. Thus by adding replacing the bids for $S_c\cup \{r\}$ with $y_{S_c\cup \{r\}}^g$, the learned model will not be severely influenced. \note{Is it necessary to have a small experiment for these arguments?}

In $w_{b, undo}$, although the bids for $S_c\cup \{r\}=-\mathds{1}$ are fixed, the colluding group $S_c$ is still unknown. We can define the following detection criterion, in which we give an lower bound for $X_{r, p}w_{b, undo}$ from observed data $X$ and $y$:
\begin{enumerate}
	\item Solve the minimization problem:

	\begin{equation}
		\label{equ:dud_obj}
    	S^* = \argmin_{S\subseteq [m]: |S|=L_d} X_{r, p}H^{-1}\left(X_{S\cup \{r\}}^\top y_{S\cup \{r\}}' + X_{-S\cup \{r\}}^\top  (-\mathds{1})\right),
	\end{equation}
	\item Replace the bidding labels for $S^*\cup \{r\}$ by $-\mathds{1}$ which leads to a new linear model with

	$$w_{undo} = H^{-1}\left(X_{-S^*\cup \{r\}}^\top y_{-S^*\cup \{r\}} + X_{S^*\cup \{r\}}^\top (-\mathds{1})\right).$$
	\item Predict scores by $w_{undo}$. If under current linear model reviewer $r$'s rank is lower than $K$, then output \textit{true}. Otherwise, output \textit{false}.
\end{enumerate}

\begin{claim}
	$X_{r, p}w_{undo} \leq X_{r, p}w_{undo, b}$.
\end{claim}

This \emph{undo} criterion gives the guarantee that $X_{r, p}w_{undo} \leq X_{r, p}w_{undo, b} \approx X_{r, p}w_{b}$. Again, because larger scores and higher ranks have high correlation, if $r$ should have been ranked lower than $K$ under $w_{b}$, the rank of $r$ under $w_{undo}$ will most likely be lower than $K$.

\paragraph{Comparison between \emph{worst case} and \emph{undo}.} As discussed for $\emph{worst case}$, it can almost guarantee that all adversaries, whose original rank is lower than $K$, will be detected as cheaters, i.e. TPR $\approx 1$. However, in the analysis of $\emph{undo}$, since the assumption that $X_{r, p}w_{undo, b} \approx X_{r, p}w_{b}$ is data-dependent and cannot be estimated since we cannot know what the genuine bids are, the TPR for \emph{undo} may be signficantly lower than that of \emph{worst case}.

On the other hand, the following claim tells us $\emph{worst case}$ is a more aggressive than $\emph{undo}$. This implies $\emph{undo}$ will have smaller FPR.
\begin{claim}
	$X_{r, p}w_{detect} \leq X_{r, p}w_{undo}$.
\end{claim}
Notice that the quality of final assignment depends heavily on the detection FPR. If FPR is too high, many legitimate pairs will be removed from the candidates set and will deteriorate the assignment algorithm's performance. Thus we may expect that under \emph{undo}, we will have better quality of final assignment result. We will evaluate the trade-off between TPR and FPR in the experiment section.
\end{comment}

\paragraph{Detection framework.} Given both the relevance scoring model and the detection heuristic, we may instantiate our robust assignment algorithm in Algorithm \ref{alg:framework}. There are two desirable properties of the final assignment:
\begin{enumerate}[1.]
\item Each paper should be assigned to a sufficient number of reviewers that have the expertise and have expressed a willingness to review. In order to achieve this goal, the relevance scoring model must be able to learn a general relationship between reviewer-paper pair features and bids. The candidate set of reviewers after the detection phase must also contain a sufficient number of qualified reviewers, \emph{i.e.}, the detection algorithm has a low false positive rate (FPR).
\item The final assignment should be robust against collusion attacks. This goal depends on the detection algorithm's ability to detect the majority of malicious reviewers and remove them from the candidate set, \emph{i.e.} it has a high true positive rate (TPR).
\end{enumerate}
The trade-off between FPR and TPR for a detection algorithm is inherent. Given the aggressive nature of the \critonelong{} heuristic, we expect that it will achieve a perfect TPR when $M_c \leq M_d$ but also has a very high FPR. In contrast, \crittwolong{} should achieve a relatively low FPR but its TPR should be lower than that of \critoneshort{}. The empirical behavior of these detection heuristics is dependent on the specific conference and may vary across different reviewers and papers. We will present a detailed study into this trade-off in section \ref{sec:experiment}.

\begin{comment}
\subsection{Criteria}
\begin{algorithm}[!htbp]
\label{algo: cre2}
\SetAlgoLined
\textbf{Input:}$r$, $p$, $K$, $L$, $H_{inv}$, $y_{train, -r}$, $X_{train, -r}$, $X_{train, r}$, $X_{p}$.\;
    $S_{\mathbf{adv}}, y_{\mathbf{adv}, S_{\mathbf{adv}}\cup\{r\}} = \arg\min_{y_r\in C; |S|=L; \forall r'\in S, y_r'\in C} X_{p, r}H_{inv}\left(X_{train, S\cup \{r\}}^Ty_{S\cup \{r\}} + X_{train, -S\cup \{r\}}^T y_{train, -S\cup \{r\}}\right)$ where the constraint $C=\{v\in \{-3, -1, 3\}^n: \text{both the number of -3 and 3 occur at most 25 times in $v$}\}$\;
    $advRank = rank\left(X_{train, S_{\mathbf{adv}}\cup \{r\}}^Ty_{\mathbf{adv},  S_{\mathbf{adv}}\cup\{r\}} + X_{train, -S_{\mathbf{adv}}\cup \{r\}}^T y_{train, -S_{\mathbf{adv}}\cup \{r\}}\right)$\;
    \eIf{$advRank > K$}{
    \textbf{Return} True\;
    }{
    \textbf{Return} False\;
    }
 \caption{CheatingCriterionApprox($r$, $p$, $K$, $L$, $H_{inv}$, $y_{train, -r}$, $X_{train, -r}$, $X_{train, r}$, $X_{p}$): Approximate Criterion to detect cheating event}
\end{algorithm}

\begin{algorithm}[!htbp]
\label{algo: cre3}
\SetAlgoLined
\textbf{Input:}$r$, $p$, $K$, $L$, $H_{inv}$, $y_{train, -r}$, $X_{train, -r}$, $X_{train, r}$, $X_{p}$.\;
    $S_{\mathbf{adv}} = \arg\min_{|S|=L} X_{p, r}H_{inv}\left(X_{train, S\cup \{r\}}^Ty_{S\cup \{r\}} + X_{train, -S\cup \{r\}}^T (\mathbf{-1})\right)$\;
    $advRank = rank\left(r, X_p H_{inv}(X_{train, -r\cup S_{\mathbf{adv}}}^Ty_{train, -r\cup S_{\mathbf{adv}}} + X_{train, -S_{\mathbf{adv}}\cup \{r\}}^T (\mathbf{-1})\right)$\;
    \eIf{$advRank > K$}{
    \textbf{Return} True\;
    }{
    \textbf{Return} False\;
    }
 \caption{CheatingCriterionUndo($r$, $p$, $K$, $L$, $H_{inv}$, $y_{train, -r}$, $X_{train, -r}$, $X_{train, r}$, $X_{p}$): Approximate Criterion to detect cheating event}
\end{algorithm}

\subsection{Paper assignment with detections}
\end{comment}


==> sections/impact.tex <==
%!TEX root=../neurips_main.tex
\section*{Broader Impact}
\label{sec:impact}

Automated paper assignment is an important component of modern conference management that is used in many top computer science conferences.
The attacks we study in this paper are modeled after realistic threats to the integrity of these conferences.
Indeed, there is anecdotal evidence that some reviewers have attempted to alter paper assignments using similar attacks.
Such alterations can be achieved by posting their paper in private chat groups and propose a \emph{quid pro quo}, or by pressuring junior researchers to bid on a particular paper and provide a positively biased review. 
Our paper seeks to better understand and recognize such attacks.
However, it does not provide a mechanism to prove beyond a reasonable doubt that an attack occurred.
We include a warning in our code base that our detection of adversarial reviewers does not provide any proof of wrongdoing.

With security papers like ours, there is always a risk that publication of the paper may encourage adversaries to stage the attacks described therein.
We have considered this risk but think it is important to publish our paper anyway because security-by-obscurity does not provide actual security.
Importantly, our paper proposes a practical defense against attacks that can be used to prevent bidding manipulation from happening in future conferences.
As a result, we believe that our work can have positive impact on the quality of the review process of scientific conferences.


==> sections/intro_old.tex <==
\section{Introduction}

Peer-reviewing, which dates to the $18^{\text{th}}$ century, forms the cornerstone of the research publication model for areas spanning from arts, sciences, humanities, social sciences and beyond. The peer-review process is mandated with a task that requires (i) maintaining objectivity, unbiasedness and transparency while (ii) performing a rigorous evaluation by {\em qualified} reviewers to ensure only research contributions that meet a sufficient acceptance threshold are allowed to be presented as a part of proceedings of a conference/journal. It is therefore of the utmost importance to select appropriate reviewers with recognized expertise who are unbiased towards the paper under review.

Due to a sharp rise in the number of papers that are submitted to a typical CS conference venue (and specifically, to a machine learning venue such as NeurIPS~\citep{charrez2019neurips}), most organizers have opted for an automated paper assignment procedure powered by a reviewer bidding phase, where, a reviewer exercises his/her preference towards reviewing papers that they are particularly interested in.
%In these systems, a combination of the bids, expert judgements (quantifying a paper-reviewer match) as well as an automated Machine Learning model's judgement of a paper-reviewer match is used to generate a final score which is fed into an assignment algorithm that presents final reviewer assignments for each paper. These systems have served the CS research community in largely positive ways (refer to the related work section for more details in this regard).
Despite the fact that these systems have served the CS research community in largely positive ways, they tend to show vulnerability towards anomalous bidding patterns of the reviewers. In particular, a group of reviewers may be incentivized to collectively bid on a certain paper, whose author may be a friend or acquaintance that reciprocates the favor to mutually benefit from the act.
%which leads us to the following question: ``are our current paper-assignment systems robust in the presence of bad actors, and in particular, when (colluding) reviewers who use their bids in order to get certain papers (which they rightfully are not mandated to review) assigned to themselves?''
We show that current paper-bidding systems exhibit a great degree of vulnerability towards manipulated bids of such reviewers (refer to Figure~\ref{fig:prob_motivate} in section~\ref{sec:motivation} for details).

Motivated by this serious shortcoming, we design and analyze a paper-bidding and assignment process that is robust towards malicious reviewers and ensures fair assignment for all papers. We first train a supervised learning model for predicting the bid of a reviewer for a given paper given the features of a paper-reviewer pair. This model serves the purpose of capturing the typical reviewer's bidding behavior. Furthermore, assuming that the vast majority of reviewers bid with no ulterior motives, we formulate a training data anomaly detection problem for identifying (colluding) reviewers whose bidding pattern is suspicious and atypical, and subsequently remove their preferences (logged during the bidding process) towards reviewing certain papers.  We evaluate our system against a white-box adversary, whose knowledge of the system and of other reviewers far exceeds that of any practically admissible attack, and show that we can achieve a very high detection rate without sacrificing assignment quality.

In summary, the contributions of our paper are as follows:
\begin{enumerate}[1.]
\item We evaluate a sample assignment system and show that malicious reviewers can gain a substantial advantage over others by colluding to bid on a single target paper.
\item We propose a robust paper assignment framework that detects malicious reviewers and removes them from the final assignments. Our framework learns the proper bidding behavior from the collected bids and marks abnormally influential training instances as potentially malicious.
\item We demonstrate empirically on a real conference dataset that our framework can achieve a high detection rate against collusion attacks, even if the adversary has full knowledge of our assignment system and the features and bids of all reviewers.
\item Finally, we evaluate several quality metrics and show that our detection framework does not compromise the assignment quality for honest reviewers.
\end{enumerate}

%Now, given how widespread bidding based paper assignment systems feature in the Computer Science conference publishing venues, this significant vulnerability of paper assignment systems requires to be addressed in order to ensure a robust and fair paper assignment process. This security issue of current paper-bidding systems motivates the core of this paper's contributions, which is to design a paper-bidding process that is robust towards detecting and marginalizing corrupted bids by reviewers and ensure that the resulting system presents a fair paper-assignment process for all papers submitted to a given conference venue.

%This paper's first contribution is to learn the bidding behavior of a {\em typical} reviewer. Now, assuming that the vast majority of reviewers bid with no ulterior motives, the average bidding pattern of a reviewer can be estimated by training a supervised Machine Learning model that takes as inputs the features from a paper-reviewer pair and uses the bid on a given paper-reviewer pair as targets. Given that most reviewers bid on about $25-50$ papers, this Machine Learning model can be learnt in robustly owing to a large quantity of available labeled data. Learning this bidding pattern of a typical reviewer presents us with an ability to not take every bid of (each) reviewer at face value (i.e. as gold standard). Instead, this Machine Learning model enables us to probe into the question as to whether a given reviewer (or a given set of (colluding) reviewers) conforms to the {\em typical} bidding pattern or not. Answering this detection question accurately enables us to sift through bidding patterns of reviewers in order to detect a potentially small subset of reviewers who may not conform to this typical bidding pattern. Re-training the resulting model on reviewers adhering to reasonably conformant behavior patterns allows us to generate preference scores for every paper-reviewer pair that can be fed into an assignment algorithm to generate final reviewing assignments.

%In essence, this paper not only attempts to learn a strong model of reviewer bidding preferences, but also presents a modeling strategy that allows us to (a) {\em efficiently} evaluate a variant of a whitebox data poisoning attack that is employed by a set of (colluding) reviewers to target a specific paper to be assigned to them. This attack is stronger than any practially admissible (blackbox) variant of the attack, (b) this modeling framework allows for the design of two detection mechanisms that is used to identify a set of colluding reviewers and which straddle different regimes of the TPR vs. FPR tradeoff. We present empirical evidence towards these claims by working with the CENSORED bidding data. More formally, following are the contributions of this paper:

\iffalse
In late $2000$'s, the field of Machine Learning experienced a surge in interest and (more critically) in the number of submissions which tended to exceed a thousand or so for a top conference venue (such as ICML/NeurIPS) in a single year. This led to the creation of the automated paper-reviewer matching system dubbed the Toronto Paper Matching System (TPMS)~\citep{charlin2013toronto} (and followed up by several others including EasyChair, HotCRP - we will focus on the case of TPMS in this paper). TPMS sought to offset the struggles associated with manually matching papers with appropriate ``expert'' reviewers in order to uphold the mandates of the reviewing process. In a nutshell, the TPMS pipeline first generates a score for a reviewer-paper pair (as measured through his/her prior publications). This score is then combined with an area chair's feedback as well as the reviewer's own bids (which is used to signal interest in reviewing a paper, but not necessarily signifying expertise of the reviewer) to generate a final score for a given paper-reviewer pair. These final scores, aggregated over all paper-reviewer pairs is then fed to an assignment algorithm that finally presents an assignment. To a great extent, the TPMS procedure has served the community tremendously over the past few years, considering the surge in number of submissions (that appears to grow exponentially) and hit nearly a nine thousand submissions or more for every conference venue over the past year. Despite these overwhelmingly large positive views of paper bidding systems (including TPMS), the growth of areas allied with Machine Learning and more broadly, Artificial Intelligence has led to several issues with the standard TPMS system - we defer a more detailed description of this to the related work section.

%Despite the largely positive effect of automating the paper-reviewer assignment process, there have been several studies on paper matching systems that detail issues including (a) assigning for some papers all relevant reviewers, whereas for other papers, assigning all irrelevant reviewers (which has a determental impact on its review quality), (b) unfair assignments (in the sense of reviewer matching) for interdisciplinary papers. This has led to several recent advancements that tend to provide fair and balanced assignments, improve the bidding process (that is used in part to generate scores for assignment) so as to make it fairer across papers. \rk{need to cite based on Nihar's presentation} \cg{is this part necessary in the intro or better fits into related works?}

Despite all these advances, given the heavy reliance of automated paper-bidding systems such as TPMS on an underlying Machine Learning model that computes similarity scores on paper-reviewer pairs (as described above) \cg{there is no learning involved yet}, it is important to consider whether there are variants of data poisoning attacks that tend to affect Machine Learning systems in general also have an impact on the functioning of TPMS based systems \cg{will it cause confusion to refer to this pipeline as the TPMS system?}. In particular, can a TPMS system be influenced by one or more bad actors (which in this case can be reviewers) who can collude with each other and alter their bids so that a paper (or a set of papers) can be assigned to them? Considering the case of CENSORED $2018$ papers, it is possible to design an efficient attack that can alter the assignment of $a\%$ papers to be assigned to a particular reviewer. Refer to section~\ref{sec:motivation} for more details. This experiment highlights the necessity towards developing paper assignment systems and procedures (that can potentially build off of existing systems) that require to be resilient and secure towards such attacks.

In order to make progress towards a robust paper matching system which functions even in the presence of a (potentially) small group of malicious actors, this paper considers a sample paper matching system employed in CENSORED-$2018$. We perform some changes to the loss function that allows us to be amenable to evaluating and detecting attacks potentially employed by a set of bad actors on the system (in order to get access to a specific paper to review). In particular, we consider the linear least squares regression objective to learn a model of the preferences of paper-reviewer pairs, and this works similar to the system employed in CENSORED-$2018$ in terms of the various metrics that we measure. Next, we demonstrate that this system is very much vulnerable to the presence of multiple colluding bad actors (\emph{i.e.}, reviewers), who can stand to gain a great advantage towards getting access to a specific paper by appropriately changing their bidding patterns. We present theoretical evidence towards the claim that the attack we simulate is the worst that can be used to influence the assignments. Despite this (worst-case) attack, given the nature of our objective, we propose a framework that detects such malicious actors and removing their influence in order to generate the final set of assignments. Empirically, we demonstrate that the defense framework proposed by this paper presents strong performance despite the worst-case nature of the attack on the system using data from the CENSORED-$2018$ conference.
\fi


%The peer-reviewing process faces the difficult job of having to straddle the fine line between maintaing objectivity, unbiasedness and transparency of judging a research contribution while simultaneously ensuring the high quality and novelty necessitated for ensuring the publication of a research contribution. This tension tends to place a heavy strain on the peer-review process,


%Owing to the basic requirements of maintaining an unbiased judgement, objectivity, transparency in the publication process, as well as with an aim towards requiring to uphold a high quality of publications, the peer-review process tends to often be an area that places a significant strain on the publication process%Peer-reviewing turns out to be an aspect that places significant strain on the research publication pipeline, owing to its importance in guaranteeing an unbiased, yet a robust means towards vetting

\iffalse
Commonly at the begining of the reviewing process of artificial intelligence conferences \fw{or peer-review conferences?}, the reviewers can read the titles and abstracts of all paper submissions and bid a subset of them.
The program chair then assign each paper to several reviewers based on the bids as well as the expertices of the reviewers.
Specifically, each paper would be assigned to one of the area chairs and at least three reviewers.
However, as field grows rapidly, we observe an expotial increase in the total submissions.
For examples, the total submissions in NeurIPS grows from 1838 papers in 2015, 2403 papers in 2016, to 6743 papers in 2019.
With such enormous number of papers, it is almost impossible to assign the papers by hands.
Recently, program chairs employ machine learning models~\citep{charlin2013toronto} to match papers with relevent reviewers assign the paper based on area chairs' suggestions as well as some algorithms.

\rk{Introduction pointers:}
Introduce the problem of paper bidding:
\begin{itemize}
	\item cite TPMS, Nihar Shah and other people's papers. Talk about the fact that many different approaches have been considered including (a) developing better assignment approaches, (b) improving various diversity related issues in the bidding process (e.g. ensuring both experts as well as intermediate levels of reviewers bid on a given paper).
	\item This paper considers issues relating to security and robustness of the paper bidding process, especially considering issues such as co-ordinated bidding amongst reviewers to get assigned specific papers - ask Kilian about how to cite these issues.
	\item Give a broad overview of the paper's approach - including, mentioning an overview of the system used in CENSORED (to give us credence for pursuing our study using this specific machine learning model), and our modifications, the use of least squares and how this design choice affects several analyses downstream without compromising loss in perf, then the defense, and relegate the details to the subsequent sections.
\end{itemize}

%Before getting to this paper's contributions, let us consider the robustness of the paper bidding process through a simple process of a collusion between (say), 3 reviewers. Draw plots of how the rank of a paper can actually go to the top-30 or so for the colluding reviewers, and say that this is sufficient for the paper to have sufficient chance of being assigned by the resulting assignment algorithm.

Round up with contributions of the paper in bullets.
\paragraph{Contributions:} (i), (ii), (iii)
\fi


==> sections/overview_notes.tex <==
\iffalse
\rk{Notes about paper organization:}

\paragraph{Section 2. Black-box attack on existing systems.}
Describe a generic scoring and assignment system, citing TPMS/Neil Lawrence. Design black-box attacks against this system and show results to instantiate our claim on need for security.\\

\paragraph{Section 3. Scoring model and detection}
3.1 Introduce notations: input features, reviewers, papers, outputs etc.\\
3.2 Describe the scoring model and loss function. Say that a variant of this system was used in AAAI and we compare how these systems perform in the experiment section. The model also provides some implicit robustness against attacks because it learns from the population about genuine bids. \\
3.3 Describe the threat model, e.g. modifying only bids, colluding attack, starting rank below 30. \\
3.4 Get to the detection and specify how it works for our specific linear model with the least squares loss.\\

\paragraph{Section 4. Problem setup:}
4.1 Describe the black-box attack for this scoring model.\\
4.2 Describe the white-box attack. We can point out that executing the white-box attack is computationally hard and give the appropriate relaxation to optimize score instead. Give some analysis regarding the different criteria.

\paragraph{Section 5: Experimental Results.}
First talk about the feature design. Also, compare against the system used in AAAI -- these differences (VW, log loss) etc. will be shown to me insignificant through validation. \rk{Maybe we can motivate the features that we use as some kind of a explicit quadratic kernel - so that the paper is using some kind of a kernel ridge regression where the kernel is the quadratic kernel?}\\

\fi
